Resynchronized Uniformization and Definability Problems for Rational Relations

Regular synchronization languages can be used to define rational relations of finite words, and to characterize subclasses of rational relations, like automatic or recognizable relations. We provide a systematic study of the decidability of uniformization and definability problems for subclasses of rational relations defined in terms of such synchronization languages. We rephrase known results in this setting and complete the picture by adding several new decidability and undecidability results.

==> figures/fig-intro.tex <==
\begin{figure}[t]
\centering
  \begin{tikzpicture}[thick,node distance=4em]
    \tikzstyle{every state}+=[inner sep=4pt, minimum size=3pt];
    \node[state, initial, initial text=$\mathcal A$] (0) {};
    \node[state, above right of= 0,yshift=-0.5cm] (1) {};
    \node[state, below right of= 0,yshift=0.5cm] (2) {};
    \node[state, accepting, below right of= 1,yshift=0.5cm] (3) {};
    \node[state, accepting, right of=3]       (4) {};
    \draw[->] (0) edge                node[]        {$d$} (1);
    \draw[->] (0) edge                node[swap]  {$e$} (2);
    \draw[->] (1) edge[loop above]    node        {$a$} ();
    \draw[->] (1) edge                node[]        {$b$} (3);
    \draw[->] (2) edge[loop above]    node        {$a$} ();
    \draw[->] (2) edge                node[swap]  {$c$} (3);
    \draw[->] (3) edge[loop above]    node        {$a$} ();
    \draw[->] (3) edge                node        {$d,e$} (4);
    \draw[->] (4) edge[loop above]    node        {$d,e$} ();

    \begin{scope}[xshift=6.5cm]
    \node[state, initial, initial text=$\mathcal U$] (0) {};
    \node[state, above right of= 0,yshift=-0.5cm] (1) {};
    \node[state, below right of= 0,yshift=0.5cm] (2) {};
    \node[state, accepting, below right of= 1,yshift=0.5cm] (3) {};
    \node[state,  right of=3]       (4) {};
    \draw[->] (0) edge[loop above]    node        {$a$} ();
    \draw[->] (0) edge                node[]        {$b$} (1);
    \draw[->] (0) edge                node[swap]  {$c$} (2);
    \draw[->] (1) edge                node[]        {$d$} (3);
    \draw[->] (2) edge                node[swap]  {$e$} (3);
    \draw[->] (3) edge[bend left]     node        {$a$} (4);
    \draw[->] (4) edge[bend left]     node        {$d$} (3);   
    \end{scope}
   \end{tikzpicture}
  \caption{
   Cf.~\cref{ex:intro};
   $S = L(\mathcal A)$ and $U = L(\mathcal U)$, we have $\llbracket U \rrbracket \subseteq_\mathsf{u} \llbracket S \rrbracket$.
   }
 \label{fig:intro}
\end{figure} 

